Zero-pairing limit of Hartree-Fock-Bogoliubov reference states

The variational Hartree-Fock-Bogoliubov (HFB) mean-field theory is the starting point of various (ab initio) many-body methods dedicated to superfluid systems. While taking the zero-pairing limit of HFB equations constitutes a text-book problem when the system is of closed-(sub)shell character, it is typically, although wrongly, thought to be ill-defined whenever the naive filling of single-particle levels corresponds to an open-shell system. The present work demonstrates that the zero-pairing limit of an HFB state is mathematically well-defined, independently of the closed- or open-shell character of the system in the limit. Still, the nature of the limit state strongly depends on the underlying shell structure and on the associated naive filling reached in the zero-pairing limit for the particle number A of interest. All the analytical findings are confirmed and illustrated numerically. While HFB theory has been intensively scrutinized formally and numerically over the last decades, it still uncovers unknown and somewhat unexpected features. From this general perspective, the present analysis demonstrates that HFB theory does not reduce to Hartree-Fock theory even when the pairing field is driven to zero in the HFB Hamiltonian matrix.

==> newcommand.tex <==
% Spherical indices
\newcommand{\nljmt}[1]{\ensuremath{n_{#1} \pi_{#1} j_{#1} m_{#1} t_{#1}}}
\newcommand{\nidx}[2]{\ensuremath{n_{#1} ljt_{#2}}}
\newcommand{\ljt}[1]{\ensuremath{ljt_{#1}}}

% Reduced matrix elements
\newcommand{\mered}[3]{\ensuremath{{{\tilde#1}}^{(\pi j t)_{#3}}_{n_{#2}n_{#3}}}}
\newcommand{\meredsup}[4]{\ensuremath{{{\tilde#1}}^{(\pi j t)_{#3} #4}_{n_{#2}n_{#3}}}}
\newcommand{\meredd}[3]{\ensuremath{{{\tilde#1}}^{(\pi j t)_{#2}}_{n_{#2}n_{#3}}}}
\newcommand{\mereddsup}[4]{\ensuremath{{{\tilde#1}}^{(\pi j t)_{#2} #4}_{n_{#2}n_{#3}}}}
\newcommand{\meredred}[4]{\ensuremath{{{\tilde#1}}^{(\pi j t)_{#4}}_{n_{#2}n_{#3}}}}
\newcommand{\meredredsup}[5]{\ensuremath{{{\tilde#1}}^{(\pi j t)_{#4} #5}_{n_{#2}n_{#3}}}}
%\newcommand{\Mered}[4]{\ensuremath{{\tilde#1}^{(\pi_{#2} j_{#2} t_{#2})}_{n_{#3};n_{#4}}}}

% Kronecker delta
\newcommand{\kd}[3]{\ensuremath{\delta_{#1_{#2}#1_{#3}} }}
\newcommand{\skd}[2]{\ensuremath{\delta_{{\tilde #1} {\tilde #2}} }}
\newcommand{\ljtkd}[2]{\ensuremath{\delta^{\ljt{#1}}_{\ljt{#2}}}}

% Angular momentum coupling
\newcommand{\jhat}[1]{\ensuremath{\hat {#1}}}
\newcommand{\clebsch}[6]{\begingroup\setlength{\arraycolsep}{0.1em}\left(\hskip -\arraycolsep\begin{array}{cc|c} #1 & #3 & #5 \\ #2 & #4 & #6 \end{array}\hskip -\arraycolsep\right)\endgroup}
\newcommand{\threej}[6]{\begingroup\setlength{\arraycolsep}{0.1em}\left(\hskip -\arraycolsep\begin{array}{ccc} #1 & #3 & #5 \\ #2 & #4 & #6 \end{array}\hskip -\arraycolsep\right)\endgroup}
\newcommand{\sixj}[6]{\begingroup\setlength{\arraycolsep}{0.2em}\begin{Bmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \end{Bmatrix}\endgroup}              
\newcommand{\ninej}[9]{\begingroup\setlength{\arraycolsep}{0.2em}\begin{Bmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{Bmatrix}\endgroup}

% Prime
\newcommand{\pr}{\prime}
\newcommand{\ppr}{{\prime\prime}}
\newcommand{\pppr}{{\prime\prime\prime}}
\newcommand{\mpr}{{M^\pr}}
\newcommand{\mppr}{{M^\ppr}}
\newcommand{\jpr}{{J^\pr}}
\newcommand{\jppr}{{J^\ppr}}
\newcommand{\kpr}{{k^\pr}}
\newcommand{\kppr}{{k^\ppr}}

% Single-particle operators
\newcommand{\spc}[1]{c^\dagger_{#1}}
\newcommand{\spa}[1]{c_{#1}}

% Braket
\newcommand{\bracket}[2]{{\langle #1 |  #2 \rangle}}
\newcommand{\bracketp}[3]{{\langle #1 |  #2 | #3 \rangle}}

%%%%% ALEX

\newcommand{\redme}[5]{\ensuremath{\tilde{#1}^{#2 (ljt)_{k_{#3}}}_{n_{k_{#4}} n_{k_{#5}}}}}
\newcommand{\redmephi}[5]{\ensuremath{\redme{#1}{#2}{#3}{#4}{#5}(\varphi)}}
\newcommand{\redmephieta}[5]{\ensuremath{\redme{#1}{#2}{#3}{#4}{#5}(\varphi,\eta)}}
\newcommand\bbone{\ensuremath{\mathbbm{1}}}
\newcommand{\elem}[2]{\ensuremath{{}^{#2}\text{#1}}}

%newcommands for J coupling section
\newcommand{\tbd}[1]{\textcolor{red}{#1}}
\newcommand{\psiref}{\vert \psi_\text{ref} \ra }
\newcommand{\den}[2]{\ensuremath{\epsilon^{#1}_{#2}}}
\newcommand{\perm}[2]{\ensuremath{\text{P}^{#1}_{#2}}}

% Omega Matrix Element
\newcommand{\ome}[5]{\Omega^{#1}_{k_{#2} k_{#3} k_{#4} k_{#5}} }
\newcommand{\omej}[6]{ {^{#6} \Omega^{#1}_{\tilde k_{#2} \tilde k_{#3} \tilde k_{#4} \tilde k_{#5}} }}


\newcommand{\emb}[1]{\ensuremath{I_{#1}}}


% model space truncation
\newcommand{\emax}{\ensuremath{e_{\text{max}}}}
\newcommand{\Emax}{\ensuremath{e_{\text{max}}}}
\newcommand{\spdim}{\ensuremath{\mathcal{D}_{SP}}}

\newcommand{\qpc}[1]{\ensuremath{\beta^\dagger_{#1}}}
\newcommand{\qpa}[1]{\ensuremath{\beta_{#1}}}
\newcommand{\qpat}[1]{\ensuremath{\tilde \beta_{{\tilde #1},-m_{#1}}}}
%\newcommand{\cre}[1]{\ensuremath{c^\dagger_{#1}}}
\newcommand{\an}[1]{\ensuremath{c_{#1}}}
\newcommand{\Ured}[2]{\ensuremath{\mathfrak{U}^{#1}_{#2}}}
\newcommand{\Vred}[2]{\ensuremath{\mathfrak{V}^{#1}_{#2}}}
\newcommand{\tr}{\ensuremath{\text{Tr}}}
\newcommand{\nljt}[1]{\ensuremath{n_{#1} \pi_{#1} j_{#1} t_{#1}}}
\newcommand{\mefull}[3]{\ensuremath{#1_{\nljmt{#2};\nljmt{#3}}}}

\newcommand{\redop}[1]{\ensuremath{{\tilde{#1}}}}

\newcommand{\sph}[1]{\ensuremath{{\tilde {#1}}}}

\newcommand{\ra}{\rangle}
\newcommand{\la}{\langle}
\newcommand{\HFB}{|\Phi \ra}
\newcommand{\qpexk}[1]{|\Phi^{#1}\ra}
\newcommand{\qpexb}[1]{\la\Phi^{#1}|}


% anti-symmetrix matrix elements
%\newcommand{\ame}[2]{\ensuremath{\la #1 \vert\vert #2\ra}}
\newcommand{\ame}[2]{\ensuremath{\la #1 \vert \hat H^{[2]} \vert #2\ra}}
\newcommand{\ameoneb}[2]{\ensuremath{\la #1 \vert \hat H^{[1]} \vert #2\ra}}
%j-coupled me
\newcommand{\jcme}[3]{\ensuremath{ {^{#3} v}_{#1,#2}}} 

% reduced matrix elements
\newcommand{\meopred}[4]{\ensuremath{{\tilde#1}^{ \, (\pi j t)_{#2} }_{n_{#3};n_{#4}} }}
% auxiliary coupled matrix element with implicit m-dependence
\newcommand{\mecaux}[4]{\ensuremath{V^{J(\pi_{#1}\pi_{#2})(t_{#1}+t_{#2})}_{\nljmt{#1}\nljmt{#2};\nljmt{#3}\nljmt{#4}}}}

%Kronecker Delta for 2B ME parity, isospin and m quantum number conditions
\newcommand{\kdMEp}[4]{\ensuremath{\delta_{(\pi_{#1}\pi_{#2})(\pi_{#3}\pi_{#4})}}}
\newcommand{\kdMEt}[4]{\ensuremath{\delta_{(t_{#1}+t_{#2})(t_{#3}+t_{#4})}}}
\newcommand{\kdMEm}[4]{\ensuremath{\delta_{(m_{#1}+m_{#2})(m_{#3}+m_{#4})}}}

% angular momentum coupling
\newcommand{\Xsym}[6]{\begingroup\setlength{\arraycolsep}{0.2em}\begin{Bmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \end{Bmatrix}_{\text{X}}\endgroup}
\newcommand{\hob}[6]{\langle\!\langle #1,#2\mspace{4mu}|\mspace{4mu}#3,#4 {\vcentcolon} #5\rangle\!\rangle_{#6}}


\newcommand{\ntidx}[2]{\ensuremath{n_{#1} lj_{#2}}}

\newcommand{\kdV}[3]{\ensuremath{\delta_{#1_{#2}-#1_{#3}} }}

\newcommand{\sphericalkd}[2]{\ensuremath{\kd{\pi}{#1}{#2} \kd{j}{#1}{#2}\kd{t}{#1}{#2}}}
\newcommand{\sktilde}[2]{\ensuremath{\delta_{\tilde #1 \tilde #2}}}

%Kronecker delta for V matrix of HFB. differs from above only in m constraint
%\newcommand{\skdV}[2]{\ensuremath{\kd{\pi}{#1}{#2} \kd{j}{#1}{#2} \delta_{m_{#1},-m_{#2}} \kd{t}{#1}{#2}}}
\newcommand{\skdV}[2]{\sktilde{#1}{#2} \delta_{m_{#1},-m_{#2}} } 

\newcommand{\uu}[1]{\underline{\underline{#1}}}
\newcommand{\Ttwo}{\ensuremath{\mathcal{T}_2}}
\newcommand{\Ttwoorder}[1]{\ensuremath{^{(#1)}\mathcal{T}_2}}

% standard line break used in align environment
\newcommand{\slb}{\notag \\ &\phantom{=} \times }
\newcommand{\slbnt}{\notag \\ &\phantom{=}  }

% reduced index
\newcommand{\redmt}[1]{\ensuremath{ \breve #1}}

% tensor notation
\newcommand{\tens}[1]{\ensuremath{ \mathcal{B}_{#1}}}
\newcommand{\tensbar}[1]{\ensuremath{ \mathcal{\bar B}_{#1}}}

\newcommand{\cre}[1]{\ensuremath{c^\dagger_{#1}}}
\renewcommand{\an}[1]{\ensuremath{c_{#1}}}

\newcommand{\Rmm}[1]{\ensuremath{R^{--}_{#1}(\varphi)}}
\newcommand{\Rmmxc}[1]{\ensuremath{\tilde R^{--}_{#1}(\varphi)}}
\newcommand{\Rmmred}[2]{\ensuremath{\tilde R^{--(ljt)_{#1}}_{n_{#1} n_{#2} }(\varphi)}}

\newcommand{\extc}{\overset{e.c.}{=}}

\newcommand{\lie}[2]{\ensuremath{\mathfrak{#1}(#2)}}

\newcommand{\qpden}[1]{\ensuremath{E_{#1}}}


\newcommand{\Vol}[1]{\ensuremath{\text{Vol}(#1)}}
\newcommand{\inftimelimit}{\ensuremath{\lim_{\tau\rightarrow \infty}}}
\newcommand{\largetimelimit}{\ensuremath{\lim_{\tau\rightarrow \infty}}}

\newcommand{\refsize}{\ensuremath{\mathcal{D}_\text{ref}}}
\newcommand{\dgr}[1]{\ensuremath{\text{deg}(#1)}}

\newcommand{\Nref}{\ensuremath{N_\text{max}^{(\text{ref})}}}

\newcommand{\norm}[1]{\ensuremath{\vert\vert #1\vert\vert}}


\newcommand{\amv}[1]{\ensuremath{ \hat{ \boldsymbol{ #1 }}}}
\newcommand{\drm}{\ensuremath{\mathrm{d}}}


